Gaussian-Flow: 4D Reconstruction with Dynamic 3D Gaussian Particle

We introduce Gaussian-Flow, a novel point-based approach for fast dynamic scene reconstruction and real-time rendering from both multi-view and monocular videos. In contrast to the prevalent NeRF-based approaches hampered by slow training and rendering speeds, our approach harnesses recent advancements in point-based 3D Gaussian Splatting (3DGS). Specifically, a novel Dual-Domain Deformation Model (DDDM) is proposed to explicitly model attribute deformations of each Gaussian point, where the time-dependent residual of each attribute is captured by a polynomial fitting in the time domain, and a Fourier series fitting in the frequency domain. The proposed DDDM is capable of modeling complex scene deformations across long video footage, eliminating the need for training separate 3DGS for each frame or introducing an additional implicit neural field to model 3D dynamics. Moreover, the explicit deformation modeling for discretized Gaussian points ensures ultra-fast training and rendering of a 4D scene, which is comparable to the original 3DGS designed for static 3D reconstruction. Our proposed approach showcases a substantial efficiency improvement, achieving a $5\times$ faster training speed compared to the per-frame 3DGS modeling. In addition, quantitative results demonstrate that the proposed Gaussian-Flow significantly outperforms previous leading methods in novel view rendering quality. Project page: https://nju-3dv.github.io/projects/Gaussian-Flow

==> sec/3dgs.tex <==
\subsection{3D Gaussian Splatting}
\label{sec:3d-splats}

\newcommand{\ADDITION}[1]{#1}
\newcommand{\REMOVAL}[1]{}
\newcommand{\CORRECTION}[2]{#2}

Our goal is to optimize a scene representation that allows high-quality novel view synthesis, starting from a sparse set of (SfM) points without normals. To do this, we need a primitive that inherits the properties of differentiable volumetric representations, while at the same time being unstructured and explicit to allow very fast rendering. We choose 3D Gaussians, which are differentiable
and can be easily projected to 2D splats allowing fast $\alpha$-blending for rendering.

Our representation has similarities to
previous methods that use 2D points~\cite{yifan2019differentiable,kopanas2021point} and assume each point is a small planar circle with a normal. 
Given the extreme sparsity of SfM points it is very hard to estimate normals. Similarly, optimizing very noisy normals from such an estimation would be very challenging.
Instead, we model the geometry as a set of 3D Gaussians that do not require normals. Our Gaussians are defined by a full 3D covariance matrix $\Sigma$ defined in world space~\cite{zwicker2001ewa} centered at point (mean) $\mu$:
\begin{equation}
	G(x)~= e^{-\frac{1}{2}(x)^{T}\Sigma^{-1}(x)}
\end{equation}
\CORRECTION{and $|\Sigma|$ is the determinant of $\Sigma$ that is a symmetric 3$\times$3 matrix}{}. This Gaussian is multiplied by $\alpha$ in our blending process.

However, we need to project our 3D Gaussians to 2D for rendering.
Zwicker et al.~\cite{zwicker2001ewa} demonstrate how to do this projection to image space. Given a viewing transformation $W$
the covariance matrix $\Sigma'$ in camera coordinates is given as follows:
\begin{equation}
	\label{eq:volume-render}
	\Sigma' = J W ~\Sigma ~W ^{T}J^{T}
\end{equation}
where $J$ is the Jacobian of the affine approximation of the projective transformation. \CORRECTION{The authors}{Zwicker et al.~\cite{zwicker2001ewa}} also show that if we skip the third row and column of $\Sigma'$, 
we obtain a 2$\times$2 variance matrix with the same structure and properties as if we would start from planar points with normals, as in previous work~\cite{kopanas2021point}.

An obvious approach would be to directly optimize the covariance matrix $\Sigma$ to obtain 3D Gaussians that represent the radiance field. However, covariance matrices have physical meaning only when they are positive semi-definite. 
For our optimization of all our parameters, we use gradient descent that cannot be easily constrained to produce such valid matrices, and update steps and gradients can very easily create invalid covariance matrices. 

As a result, we opted for a more intuitive, yet equivalently expressive representation for optimization.
The covariance matrix $\Sigma$ of a 3D Gaussian is analogous to describing the configuration of an ellipsoid.
Given a scaling matrix $S$ and rotation matrix $R$, we can find the corresponding $\Sigma$:
\begin{equation}
    \Sigma = RSS^TR^T
\end{equation}

To allow independent optimization of both factors, we store them separately: a 3D vector $s$ for scaling and a quaternion $q$ to represent rotation. These can be trivially converted to their respective matrices and combined, making sure to normalize $q$ to obtain a valid unit quaternion.

To avoid significant overhead due to automatic differentiation during training, we derive the gradients for all parameters explicitly. 
\CORRECTION{We discuss the specific case of scaling and rotation (i.e., the shape) of 3D Gaussians next.}{}
\CORRECTION{The differentiable renderer outputs 
the $2\times2$ screen-space covariance matrix $\Sigma'$.
Given the gradient of the loss $\frac{dL}{d\Sigma'}$ %
which we assume as output from the differentiable renderer, 
we can apply the chain rule to compute gradients and propagate the loss.}{}


This representation of anisotropic covariance -- suitable for optimization -- allows us to optimize 3D Gaussians to adapt to the geometry of different shapes in captured scenes, resulting in a fairly compact representation. 


Our goals are to have fast overall rendering and fast sorting to allow approximate $\alpha$-blending -- including for anisotropic splats -- and to avoid hard limits on the number of splats that can receive gradients that exist in previous work~\cite{lassner2021pulsar}.

To achieve these goals, we design a tile-based rasterizer for Gaussian splats inspired by recent software rasterization approaches~\cite{lassner2021pulsar} to pre-sort primitives for an entire image at a time, avoiding the expense of sorting per pixel that hindered previous $\alpha$-blending solutions~\cite{kopanas2021point,kopanas2022neural}. Our fast rasterizer allows efficient backpropagation over an arbitrary number of blended Gaussians with low additional memory consumption, requiring only a constant overhead per pixel. 
Our rasterization pipeline is fully differentiable, and given the projection to 2D can rasterize anisotropic splats similar to previous 2D splatting methods~\cite{kopanas2021point}.

Our method starts by splitting the screen into 16$\times$16 tiles, and then proceeds to cull 3D Gaussians against the view frustum and each tile. 
Specifically, we only keep Gaussians with a 99\% confidence interval intersecting the view frustum. 
Additionally, we use a guard band to trivially reject Gaussians at extreme positions \ADDITION{(i.e., those with means close to the near plane and far outside the view frustum)}, since computing their projected 2D covariance would be unstable.
We then instantiate each Gaussian according to the number of tiles they overlap and assign each instance a key that combines view space depth and tile ID. We then sort Gaussians based on these keys using a single fast GPU Radix sort~\cite{merrill2010revisiting}.
Note that there is no additional per-pixel ordering of points, and blending is performed based on this initial sorting.  As a consequence, our $\alpha$-blending can be approximate in some configurations. %
However, these approximations become negligible as \CORRECTION{points}{splats} approach the size of individual pixels. 
We found that this choice greatly enhances training and rendering performance without producing visible artifacts in converged scenes. 

After sorting \CORRECTION{points}{Gaussians}, we produce a list for each tile by identifying the first and last depth-sorted entry that splats to a given tile. For rasterization, we launch one thread block for each tile. Each block first collaboratively loads packets of \CORRECTION{points}{Gaussians} into shared memory and then, for a given pixel, accumulates color and $\alpha$ values by traversing the lists front-to-back, thus maximizing the gain in parallelism both for data loading/sharing and processing.
When we reach a target saturation of $\alpha$ in a pixel, the corresponding thread stops. At regular intervals, threads in a tile are queried and the processing of the entire tile terminates when all pixels have saturated (i.e., $\alpha$ goes to 1).

During rasterization, the saturation of $\alpha$ is the only stopping criterion. In contrast to previous work, we do not limit the number of blended primitives that receive gradient updates. We enforce this property to allow our approach to handle scenes with an arbitrary, varying depth complexity and accurately learn them, without having to resort to scene-specific hyperparameter tuning. 
During the backward pass, we must therefore recover the full sequence of blended points per-pixel in the forward pass. One solution would be to store arbitrarily long lists of blended points per-pixel in global memory~\cite{kopanas2021point}. To avoid the implied dynamic memory management overhead, we instead choose to traverse the per-tile lists again; we can reuse the sorted array of Gaussians and tile ranges from the forward pass. To facilitate gradient computation, we now traverse them back-to-front.

The traversal starts from the last point that affected any pixel in the tile, and loading of points into shared memory again happens collaboratively. Additionally, each pixel will only start (expensive) overlap testing and processing of points if their \CORRECTION{index}{depth} is lower than or equal to the \CORRECTION{index}{depth} of the last point that contributed to its color during the forward pass.
\CORRECTION{ Rather than storing a list of of progressively shrinking opacity values during the forward pass, we recover the values from those in the forward pass. }{Rather than trasversing an explicit list of progressively shrinking opacities in the backward pass, we can recover these intermediate opacities by storing only the total accumulated opacity at the end of the forward pass.}
Specifically, each point stores the final accumulated opacity $\alpha$ in the forward process; we divide this by each point's $\alpha$ in our back-to-front traversal to obtain the required coefficients for gradient computation.
